Discrete Diffusion Models with MLLMs for Unified Medical Multimodal Generation

Recent advances in generative medical models are constrained by modality-specific scenarios that hinder the integration of complementary evidence from imaging, pathology, and clinical notes. This fragmentation limits their evolution into foundation models that can learn and reason across the full spectrum of biomedical data. We propose MeDiM, the first medical discrete diffusion model that learns shared distributions across modalities without modality-specific components. MeDiM unifies multiple generative tasks: translating between images and text, and jointly producing image-report pairs across domains in response to prompts. Built on a discrete diffusion framework, MeDiM bridges vision and language representations through a shared probabilistic space. To enable unified and flexible medical generation, we employ a multimodal large language model (MLLM) as the diffusion backbone, leveraging its prior knowledge and cross-modal reasoning. Two key designs are introduced: (1) removing the causal attention mask for bidirectional context, and (2) injecting continuous timestep embeddings for diffusion awareness. Experiments demonstrate high-fidelity medical generation (FID 16.60 on MIMIC-CXR and FID 24.19 on PathGen) and accurate report generation (METEOR 0.2650 and 0.2580). Jointly generated image-report pairs further enhance downstream performance (plus6.43 percent BLEU-1, plus18.57 percent BLEU-2, plus31.58 percent BLEU-3, plus4.80 percent METEOR), showing that MeDiM supports coherent and clinically grounded multimodal outputs.

==> section/related_work.tex <==
\section{Related Work}

\paragraph{Medical Image Generation}
Owing to data scarcity, medical image generation is gaining increasing significance as a research focus. 
Early studies~\citep{chartsias2017adversarial,guo2020anatomic,huo2018synseg,zhang2018translating} employed GANs to augment medical imaging data, improving the performance of downstream medical tasks. 
In recent years, diffusion models~\citep{ho2020denoising,rombach2022high} have shown stable training and promising performance in high-quality image generation tasks, motivating a growing body of work to explore their application in medical image generation~\citep{mao2025medsegfactory,lyu2022conversion,chambon2022roentgen,gungor2023adaptive}. 
Fast-DDPM~\citep{jiang2025fast} and LLCM~\citep{polamreddy2025leapfrog} focus on accelerating the diffusion-based generation of medical images. 
EMIT-Diff~\citep{zhang2024diffboost} and MAISI~\citep{guo2025maisi} incorporate ControlNet~\citep{zhang2023adding} to achieve anatomically or semantically controllable medical image synthesis. 
By introducing non-linear Kolmogorov-Arnold Networks (KANs)~\citep{liu2024kan} and globally modeling Transformers~\citep{vaswani2017attention,Peebles2022DiT} as diffusion backbones, U-KAN~\citep{li2025u} and Med-Art~\citep{guo2025med} demonstrate state-of-the-art performance in generating medical images across diverse modalities, which motivates the consideration of backbone design for discrete diffusion models in MeDiM.

\paragraph{Medical Report Generation}
Medical report generation is commonly facilitated by VLMs~\citep{li2022blip,li2023blip,zeng2023conzic} endowed with domain-specific medical knowledge. 
\citet{yang2022knowledge} enhanced the medical literacy of VLMs by combining general medical background with image-specific clinical knowledge, while \citet{zhang2020radiology} designed a medical knowledge graph to further enrich medical VLMs. 
R2Gen~\citep{chen-emnlp-2020-r2gen} and R2GenCMN~\citep{chen-acl-2021-r2gencmn} generate radiology reports based on memory-driven Transformer architectures. 
\citet{chen2023fine} improved the interpretability of medical report generation by associating local medical image regions with medical terminology in the report, while \citet{liu2024factual} enhanced image–report alignment through fact-guided contrastive learning. 
RGRG~\citep{tanida2023interactive} employs region-level guidance for medical report generation, while \citet{zhang2024attribute} addresses its limitation of neglecting shared attributes for each local region via attribute prototype guidance.
\citet{liu2024bootstrapping} leveraged priors from LLMs to improve medical report generation. 
MLRG~\citep{liu2025enhanced} enhances medical visual information by integrating multiple views of the same medical image. 
However, most existing approaches are limited to specific medical report generation tasks. 
To overcome this issue, we present MeDiM, which formulates the joint discrete distribution of medical images and reports independent of imaging modalities and organ-specific characteristics.


\paragraph{Unified Multimodal Understanding and Generation}
Unified multimodal models aim to build an MLLM, modeling and reasoning over both image and textual sequences. 
Early studies~\citep{ge2307planting,ge2024seed,sun2024generative,sun2023emu,li2022blip} attempted to combine CLIP~\citep{radford2021learning}, which aligns the visual–language space, with LLMs to process images and text separately. 
Given that CLIP operates in a continuous visual space, some studies~\citep{liu2024world,team2024chameleon,wu2024vila} have explored using VQ-VAE~\citep{van2017neural} to represent visual information as discrete sequences. 
Meanwhile, numerous studies~\citep{yu2023scaling,lu2024unified,xie2024show,wu2025janus} discussed leveraging the strengths of both encoders. 
Studies such as LWM~\citep{liu2024world} and Chameleon~\citep{team2024chameleon} have shown that discrete visual features can be integrated with language tokens into a unified sequence, facilitating joint cross-modal modeling. 
Although this design obviates the need for modality-specific components, it incurs substantial training costs. 
Liquid~\citep{wu2024liquid} introduces a pre-trained LLM as the backbone to solve this issue. 
However, AR suffers from low inference efficiency.
Given the efficiency in generation and success in understanding of discrete diffusion models, UniD3~\citep{hu2022unified} and UniDisc~\citep{swerdlow2025unified} adopt them as a unified framework. 
MMaDA~\citep{yang2025mmada} further employs LLaDA~\citep{nie2025large} as the backbone for a unified discrete diffusion model. 
However, MMaDA is restricted to a single diffusion-based MLLM backbone, whereas MeDiM can leverage the wider spectrum of AR MLLM backbones, providing greater scalability.

